Transition Transfer $Q$-Learning for Composite Markov Decision Processes

To bridge the gap between empirical success and theoretical understanding in transfer reinforcement learning (RL), we study a principled approach with provable performance guarantees. We introduce a novel composite MDP framework where high-dimensional transition dynamics are modeled as the sum of a low-rank component representing shared structure and a sparse component capturing task-specific variations. This relaxes the common assumption of purely low-rank transition models, allowing for more realistic scenarios where tasks share core dynamics but maintain individual variations. We introduce UCB-TQL (Upper Confidence Bound Transfer Q-Learning), designed for transfer RL scenarios where multiple tasks share core linear MDP dynamics but diverge along sparse dimensions. When applying UCB-TQL to a target task after training on a source task with sufficient trajectories, we achieve a regret bound of $\tilde{O}(\sqrt{eH^5N})$ that scales independently of the ambient dimension. Here, $N$ represents the number of trajectories in the target task, while $e$ quantifies the sparse differences between tasks. This result demonstrates substantial improvement over single task RL by effectively leveraging their structural similarities. Our theoretical analysis provides rigorous guarantees for how UCB-TQL simultaneously exploits shared dynamics while adapting to task-specific variations.

==> 3-regret-analysis.tex <==
\section{Regret Analysis} 

Let $N$ denote the number of samples. By Proposition 3 in \citep{basu2019low}, for $N$ large enough, \footnote{$N \succsim q \paran{\frac{\sup_{\theta \in [-\pi, \pi]}\Lambda_{\max}(f_X(\theta))}{\sup_{\theta \in [-\pi, \pi]}\Lambda_{\min}\paran{f_X(\theta)}}}^2$ where $f_X$ is the spectral density of the VAR model.} there exists a constant $C_N>0$ such that 
\begin{equation}
\Lambda_{\min}\left(\frac{{\bX}^{\top}\bX}{N}\right) \leq C_N,
\label{eq:ass-number}
\end{equation}

\begin{theorem}
$\norm{\hat\bDelta^L}_F^2+\norm{\hat\bDelta^{S}}_F^2\leq 4c_0\frac{2rd+s\log d}{\zeta N}$
\label{thm:rl-upperbound}
\end{theorem}

\begin{proof}

$\hat\bDelta^{L}=\hat\bL-\bL^*, \hat\bDelta^{S}=\hat\bS-\bS^*$

$\frac{1}{2}\norm{\bY-\bX\paran{\hat{\bL}+\hat{\bS}}}_F^2\leq\frac{1}{2}\norm{\bY-\bX(\bL^*+\bS^*)}_F^2$

$\frac{1}{2}\norm{\bX(\hat\bDelta^{L}+\hat\bDelta^{S})}_F^2\leq \angles{\bX^\top\bE, \hat\bDelta^{L}+\hat\bDelta^{S}}\leq \norm{\bX^\top \bE}_2\norm{\hat\bDelta^{L}}_*+\norm{\bX^\top \bE}_{\max}\norm{\hat\bDelta^{S}}_1$

   $\frac{1}{2}\norm{\bX\left(\hat\bDelta^L+\hat\bDelta^{S}\right)}_F^2 \geq \frac{\zeta}{2} \paran{ \norm{\hat\bDelta^L +\hat\bDelta^{S}}_F^2}
   \geq \frac{\zeta}{2} \paran{ \norm{\hat\bDelta^L}_F^2 +\norm{\hat\bDelta^{S}}_F^2}-\zeta\abs{\angles{\hat\bDelta^L ,\hat\bDelta^{S}}}
   $


   
By the separation lemma presented in \cite{chai2024structured}, this lemma demonstrates that two matrices can be well-separated to a certain extent under the incoherence assumption. Given two $\mu'$-incoherent matrices $G_1,G_2\in \RR^{p \times q}$, with $\mu'$ having an upper bound $\mu$, and $\rank(G_1),\rank(G_2)\leq r$. Let $\bDelta^G=G_1-G_2$, we have $\frac{\norm{\bDelta^G}^2_{max}}{\norm{\bDelta^G}_F^2}\leq \frac{c\mu r^4}{\max\{p,q\}}$, 
    
    Define the support sets of matrices $\hat\bDelta^{L}$ and $\hat\bDelta^{S}$ as $ \text{supp}(\hat\bDelta^{L})=\{(i,j)\mid \hat\bDelta^{L}_{i,j}\neq 0\}$ and $\text{supp}(\hat\bDelta^{S, (k)})\{(i,j)\mid \hat\bDelta^{S, (k)}_{i,j}\neq 0\}$, respectively, and let $J = \text{supp}(\hat\bDelta^{L}) \cap \text{supp}(\hat\bDelta^{S, (k)})$. The projection operator $\Pi_J$ zeros out elements not in $J$. Hence,$$\frac{\norm{\Pi_J(\hat\bDelta^{L})}_F^2}{\norm{\hat\bDelta^{L}}_F^2}\leq |J|\frac{\norm{\hat\bDelta^{L}}_{max}^2}{\norm{\hat\bDelta^{L}}_F^2}\leq 2s\frac{c\mu r^4}{\max\{p,q\}}\leq \frac{\max\{p,q\}}{8c\mu r^4}\frac{c\mu r^4}{\max\{p,q\}}=\frac{1}{4}$$
    Same to $\hat\bDelta^{S}$, $$\abs{\angles{\hat\bDelta^L,\hat\bDelta^{S}}}=\abs{\angles{\Pi_J(\hat\bDelta^L),\Pi_J(\hat\bDelta^{S})}}\leq \norm{\Pi_J(\hat\bDelta^L)}_F^2+\norm{\Pi_J(\hat\bDelta^{S})}_F^2\leq \frac{1}{4}\paran{\norm{\hat\bDelta^{L}}_F^2+\norm{\hat\bDelta^{S}}_F^2}$$

$$\frac{1}{2}\norm{\bX\left(\hat\bDelta^L+\hat\bDelta^{S}\right)}_F^2 \geq \frac{\zeta}{4} \paran{ \norm{\hat\bDelta^L}_F^2 +\norm{\hat\bDelta^{S}}_F^2},$$

    \begin{equation}
     \begin{aligned}
      &\frac{\zeta}{4} \paran{ \norm{\hat\bDelta^L}_F^2 + \norm{\hat\bDelta^{S}}_F^2 }
      \leq \norm{\bX^\top \bE}_2\norm{\hat\bDelta^L}_* + \norm{\bX^\top \bE}_{\max}\norm{\hat\bDelta^{S}}_1\\
      &
      \leq \sqrt{2r}\norm{\bX^\top \bE}_2\norm{\hat\bDelta^L}_F + \sqrt{s}\norm{\bX^\top \bE}_{\max}\norm{\hat\bDelta^{S}}_F\\
      &\leq \sqrt{ \paran{\norm{\hat\bDelta^L}_F^2 + \norm{\hat\bDelta^{S}}_F^2}\paran{2r\norm{\bX^\top \bE}_2^2+s\norm{\bX^\top \bE}_{\max}^2}}.
     \end{aligned}
     \end{equation}
     
     By combining lemma \ref{A:3}, which provides upper bounds on 
    $\norm{\bX^{\top}\bE}_2$ and $\norm{\bX^{\top}\bE}_{\max}$, we complete the proof of Theorem \ref{thm:ts-upperbounds2}.

     \begin{equation}
     \begin{aligned}
	 \quad\norm{\hat\bDelta^L}_F^2+\norm{\hat\bDelta^{S}}_F^2\leq \frac{4}{\zeta}\paran{2r\norm{\bX^\top \bE}_2^2+s\norm{\bX^\top \bE}_{\max}^2}
     \leq 4c_0\frac{2rd+s\log d}{\zeta N}.
     \end{aligned}
     \end{equation}
\end{proof}

To ensure regularity in the feature space, we introduce regularity conditions for the feature mapping.

The matrix $\boldsymbol{\Psi} =[\psi(s_1), \psi(s_2), \ldots, \psi(s_{|S|})]^T$, with entries defined by the $\psi$ features.
\begin{assumption}
For every $v \in \mathbb{R}^S$, and positive constants $C_{\psi,1}C_{\psi,2},C_\phi$, we have

\begin{enumerate}
  \item $\|\bPsi^{\top} v\|_{\infty} \leq C_{\psi,1} \|v\|_{\infty}$, $\|\bPsi^{\top} v\|_{\text{op}} \leq C_{\psi,2} \|v\|_{\infty}$,  $\forall v \in \mathbb{R}^{|\mathcal{S}|}$.
  
  \item $\|\phi(s, a)\|_2 \leq C_\phi \sqrt{p}, \quad \forall (s, a) \in \mathcal{S} \times \mathcal{A}$.
\end{enumerate}
\label{ass-recon}
\end{assumption}
    
  If $\bPsi$ is a set of sparse or highly concentrated features, then condition (1) can be replaced with a stronger alternative: $\norm{\bPsi^{\top} v}_2 \leq C_{\psi,1} \norm{v}_{\infty}$.

  \begin{theorem}
$\text{Regret}(NH) \leq 4\sqrt{2}C_{\phi}C_{M}C'NH^2\sqrt{c_0\frac{(2rd+s\log d)p}{\zeta N}}$
\label{thm:rl-theorem}
\end{theorem}

  When updating the Q-values using Equation (\ref{eq:updateQ}), we employ the range derived from Lemma \ref{lem:boundQ} as the upper confidence bound. The central idea of our approach is to leverage the error bounds of the core matrix to establish a reasonable upper limit on the Frobenius norm of the core matrix. Following this, by identifying the optimal low-rank (L) and sparse (S) components, we can effectively calculate an optimistic estimation of the Q-values.  Furthermore, Equation (\ref{eq:updateQ}) can be replaced as 
    $$Q_{n, h}(s, a) = r(s, a) + \max_{\substack{\bL,\bS \in \mathcal{B}_n}}\phi(s, a)^{\top} (\bL+\bS) \bPsi^{\top} V_{n, h+1}$$
    where $\mathcal{B}_n=\{\bL,\bS \mid \norm{\bL-\bL_n}_F^2+\norm{\bS-\bS_n}_F^2\leq \beta_M\}$, as well as let 

    $$\widetilde{\bL}_n,\widetilde{\bS}_n=\arg\max_{\substack{\bL,\bS \in \mathcal{B}_n}}\phi(s, a)^{\top} (\bL+\bS) \bPsi^{\top} V_{n, h+1}$$

    According to Theorem \ref{thm:ts-upperbounds}, with high probability, the true transition core matrix is contained within the specified confidence bound. We denote this event by $E_n = 1$; otherwise, $E_n=0$.
    
    \begin{lemma}\label{lem:optimism}
    Given any state-action pair $(s, a) \in \mathcal{S} \times \mathcal{A}$ , for each episode $n$ and decision step $h$, $E_n=1$ we have:
        $$Q_{n,h}(s, a) \geq Q_h^*(s, a)$$
    \end{lemma}
    \begin{proof}
    For all $s\in \mathcal{S}$, $a\in \mathcal{A}$. Proceeding recursively over $h$.\\
    At $h=H$, we have $Q_{n,H}=Q_H^*(s, a)=r(s,a)$. Assuming the validity for $1<h'<H$, it naturally extends to $h=h'-1$, with $V_{n,h}(s)>V_h^*(s)$ 
    \begin{align*}
     Q_{n, h}(s, a) 
     &= r(s, a) + \max_{\substack{\bL,\bS \in \mathcal{B}_n}}\phi(s, a)^{\top} (\bL+\bS) \bPsi^{\top} V_{n, h+1}\\
     &\geq r(s, a) + \phi(s, a)^{\top} (\bL^*+\bS^*) \bPsi^{\top} V_{n, h+1}\\
     &\geq r(s, a) + [P V^*_{h+1}](s, a)=Q_h^*(s, a)
    \end{align*}
   \end{proof} 

\begin{lemma}\label{lem:boundQ} 
     Let $h \in [H]$ and $n \in [N]$. $E_n=1$, With high probability,     
     $$Q_{n,h}-\paran{r(s_{n,h},a_{n,h})+[P_h V_{h+1}](s_{n,h},a_{n,h})}
     \leq 4\sqrt{2}C_{\phi}C_{M}C' H\sqrt{c_0\frac{(2rd+s\log d)p}{\zeta N}}.$$
     \end{lemma}

\begin{proof}

   \begin{align*}
   Q_{n,h} - \big(r(s_{n,h},a_{n,h}) + [P_h V_{h+1}](s_{n,h},a_{n,h})\big) 
   =& \phi_{n, h}^{\top}\left[\left(\widetilde{\bL}_{n} + \widetilde{\bS}_{n}\right) - M^*\right] \bPsi^{\top} V_{n, h+1} \\
   = &\phi_{n, h}^{\top}\left[(\widetilde{\bL}_{n}-L^*) + \left(\widetilde{\bS}_{n}-\bS^{*}\right)\right] \bPsi^{\top} V_{n, h+1}.
    \end{align*}
        Applying Hölder's inequality, the triangle inequality, and Cauchy-Schwarz inequality, we deduce the following results:
     \begin{equation}
     \begin{aligned}
     &Q_{n,h} - \left(r + [P_h V_{h+1}]\right) \\
     &\leq \norm{\phi_{n, h}^{\top}(\widetilde{\bL}_{n} - \bL^{*})}_*\norm{\bPsi^{\top} V_{n, h+1}}_{op}+\norm{\phi_{n, h}^{\top}\paran{\widetilde{\bS}_{n} - \bS^*}}_1\norm{\bPsi^{\top} V_{n, h+1}}_{\infty} \\
     & \leq \paran{C_{\psi,1}\norm{\phi_{n, h}^{\top}(\widetilde{\bL}_{n} - \bL^*)}_*+C_{\psi,2}\norm{\phi_{n, h}^{\top}\paran{\widetilde{\bS}_{n} - \bS^{*}}}_1}H \\
     & \leq \paran{C_{\psi,1}\sqrt{2r}\norm{\phi_{n, h}^{\top}}_*\norm{\widetilde{\bL}_{n} - \bL^{*}}_F + C_{\psi,2}\sqrt{s}\norm{\phi_{n, h}^{\top}}_1\norm{\widetilde{\bS}_{n} - \bS^{*}}_F}H \\
     & \leq C_{\phi}\sqrt{p}H\paran{C_{\psi,1}\sqrt{2r}\norm{\widetilde{\bL}_{n} - \bL^*}_F + C_{\psi,2}\sqrt{s}
     \norm{\widetilde{\bS}_{n} - \bS^{*}}_F} \\
     & \leq C_{\phi}\sqrt{p}H \sqrt{\paran{ \|\widetilde{\bL}_{n} - \bL^*\|_F^2 +   \|\widetilde{\bS}_{n} - \bS^{*}\|_F^2}\paran{2rC_{\psi,1}^2+sC_{\psi,2}^2}}\\
     &\leq C_{\phi}C_{M}\sqrt{p}H
     \sqrt{
     \norm{\widetilde{\bL}_n -\hat\bL_n}^2_F + 
     \norm{\hat\bL_n -\bL^*}^2_F+\paran{\norm{\widetilde{\bS}_{n} - \hat\bS_n}^2_F+\norm{\hat\bS_n - S^{*}}^2_F}} \\
     & \leq 4\sqrt{2}C_{\phi}C_{M}C' H\sqrt{c_0\frac{(2rd+s\log d)p}{\zeta N}}.
     \end{aligned}
    \end{equation}

 constant term $C_M=\sqrt{2rC_{\psi,1}^2+sC_{\psi,2}^2}$ for brevity.
\end{proof}



In calculating the regret bound, we reformulate the regret formula based on the updates to the Q-values within the algorithm and the confidence bounds of the core matrix. $\mathcal{F}_{n,h}$ is defined as the $\sigma$-field generated by all the random variables up until episode n, step h, essentially fixing the sequence $s_{1,1}, a_{1,1}, s_{1,2}, a_{1,2}, \ldots, s_{n,h}, a_{n,h}$. 
Now, we proceed to prove Theorem \ref{thm:rl-theorem}, letting 
$$\delta_{n,h} := (V_{n,h}-V_{h}^{\pi_{n}})(s_{n,h}), \quad
\gamma_{n,h} := Q_{n,h} - \left(r(s_{n,h},a_{n,h}) + [P_h V_{h+1}](s_{n,h},a_{n,h})\right).$$
\begin{align*}
\text{Regret}(NH) &= \mathbb{E}\left(\sum_{n=1}^{N} \left[ V^*(s_0) - V^{\pi_n}(s_0) \right]\right) \\
&\leq \mathbb{E}\left( \sum_{n=1}^{N}(V_{n,1}-V_{1}^{\pi_{n}})(s_0)\right) = \sum_{n=1}^{N}\mathbb{E}(\delta_{n,1}).
\end{align*}
$$\mathbb{E}(\delta_{n,1}) = \mathbb{E}(\delta_{n,1}E_n+(1-E_n)\delta_{n,1}) 
\leq \mathbb{E}(\delta_{n,1}E_n)+Hp[E_n=0].$$
where $p[E_n=0]\leq c_1\exp\paran{-c_2\log p}$, Then we have

\begin{align*}
\mathbb{E}\paran{\delta_{n,1}E_n \mid \mathcal{F}_{n,1}} =& \paran{V_{n,1} - V_{1}^{\pi_{n}}}\paran{s_{n,1}}E_n \\
\leq &Q_{n,1}\paran{s_{n,1},a_{n,1}} - V_{1}^{\pi_{n}}\paran{s_{n,1}} \\
= &\gamma_{n,1} + \paran{r\paran{s_{n,1},a_{n,1}} +[PV_{n,2}]\paran{s_{n,1},a_{n,1}}} -V_{1}^{\pi_{n}}\paran{s_{n,1}} \\
\leq &\gamma_{n,1} + \mathbb{E}\paran{\paran{V_{n,2} - V_{2}^{\pi_{n}}}\paran{s_{n,2}}E_n \mid \mathcal{F}_{n,1}} 
\leq \cdots \leq \sum_{h=1}^{H}\gamma_{n,h}\\
\leq &4\sqrt{2}C_{\phi}C_{M}C' H^2\sqrt{c_0\frac{(2rd+s\log d)p}{\zeta N}}.
\end{align*}

Then we establish the regret bound with high probability

\begin{align*}
\text{Regret}(NH) &\leq 4\sqrt{2}C_{\phi}C_{M}C'NH^2\sqrt{c_0\frac{(2rd+s\log d)p}{\zeta N}}.
\end{align*}


==> 4-tranferRL.tex <==
\section{Transfer in Reinforcement Learning} 

\subsection{Problem settings}


The system transitions to another state $s' \in \calS$ according to an unknown transition probability $\PP(s' | s, a)$, while returning an immediate reward $r(s, a)\in [0, 1]$. 
The goal of the agent is to obtain the maximal
possible return after playing for a period of time - even though she has no knowledge about the
transition probabilities at the beginning.



Now we consider transfer learning with target task $\calM^{(0)}$ and source task $\calM^{(1)}$. 
The transition probabilities of the target and source tasks are, respectively,
\begin{equation*}
    \PP^{(0)}(s' | s, a) = \phi(s, a)^\top \bM^{(0)} \psi(s'), \quad\text{and}\quad
    \PP^{(1)}(s' | s, a) = \phi(s, a)^\top\bM^{(1)}  \psi(s').
\end{equation*}

The target and source tasks are different in that the core transition matrix $\bM^{(0)} \ne \bM^{(1)}$. 
However, their similarity is defined by \begin{equation}
    \bM^{(0)} = \bL + \bS^{(0)}, 
    \quad\text{and}\quad
    \bM^{(1)} = \bL + \bS^{(1)},
\end{equation}
where $\bU \in \RR^{p \times k}$ and $\bV \in \RR^{q \times r}$ are low-rank matrices (i.e. $k\ll p$ and $r\ll q$), $\lVert \bS^{(0)} \rVert_0 = s_0$,  $\lVert \bS^{(1)} \rVert_0 = s_1$, and their difference $\bD = \bS^{(1)} - \bS^{(0)}$ satisfies $\norm{\bD}_0 = d \ll \max\{s_0, s_1\}$.
In words, the two core transition matrices $\bM^{(0)}$ and  $\bM^{(1)}$ share the same low-rank structure and differs only in their respective sparse matrix $\bS^{(0)}$ and $\bS^{(1)}$. 

We have $N_1$ episodes for the source task and $N_0$ episodes for the target task. 
In practice, $N_1 \gg N_0$ and we would like to use the source task to enhance the performance of the target task. 

we use $i$ and $h$ to index episodes and time steps of the target task, where $i \in [N_0]$ and $h \in [H]$. For the source task, $j$ and $h$ are used to index its episodes and time steps, with $j \in [N_1]$ and $h \in [H]$.
We obtain the following state-action-station transition triplet: $(s_{i, h}, a_{i, h}, s'_{i, h})$ from the target task and $(s_{j, h}, a_{j, h}, s'_{j, h})$ from the source task.
The associated features are 
\begin{equation}
\begin{aligned}
    \phi_{i, h}^{(0)} &:= \phi(s_{i, h}, a_{i, h}) \in \RR^d, & \psi_{i, h}^{(0)} &:= \psi(s'_{i, h}) \in \RR^{q}, \\
    \phi_{j, h}^{(1)} &:= \phi(s_{j, h}, a_{j, h}) \in \RR^d, & \psi_{j, h}^{(1)} &:= \psi(s'_{j, h}) \in \RR^{q}.
\end{aligned}
\end{equation}

Let $\bK_{\psi} := \sum_{s'\in\calS} \psi(s') \psi(s')^\top$. 
We have, at each step $h$, for the target task, 
   $$\EE\brackets{\phi_{i,h}\psi_{i,h}^\top \bK_{\psi}^{-1} \mid s_{i,h}, a_{i,h}} 
    = \paran{\phi_{i,h} \phi_{i,h}^\top} (\bL + \bS^{(0)})$$
    
Similarly, we have for the source task, 
$$\EE\brackets{\phi_{j,h}\psi_{j,h}^\top \bK_{\psi}^{-1} \mid s_{j,h}, a_{j,h}}= \paran{\phi_{j,h} \phi_{j,h}^\top} \bM^{(1)}= \paran{\phi_{j,h} \phi_{j,h}^\top} (\bL + \bS^{(1)})$$

\noindent{\sc Step I.} Estimate the low-rank component $\bM = \bL + \bS$ by solving\footnote{Note here that observations over $h \in [H]$ are not independent, one way to avoid this is to use non-stationary $\PP_h$, and thus $\bM_h$, for each step. 
For this moment, we will work with stationary and see if the proofs will go through with dependence over $h$.} 

We denote $Y_{i,h}=\phi_{i,h}\psi_{i, h}^{\top}K_{\psi}^{-1}$, $X_{i,h}=\phi_{i,h}\phi_{i,h}^\top$ and $Y_{j,h}=\psi_{j, h}^{\top}K_{\psi}^{-1}$, $X_{j,h}=\phi_{j,h} \phi_{j,h}^\top$

\begin{equation}
\begin{aligned}
&(\hat{\mathbf{L}}, \hat{\mathbf{S}}) \in 
    \underset{\mathbf{L}, \mathbf{S} \in \mathbb{R}^{p \times q}}{\arg\min}\;  \sum_{i^{\prime}<i, h \leq H}\left\|Y_{i,h}-X_{i,h}(\boldsymbol{L}+\boldsymbol{S})\right\|_{2}^{2}\sum_{j^{\prime}<j, h \leq H}\left\|Y_{j, h}-X_{j,h}(\boldsymbol{L}+\boldsymbol{S})\right\|_{2}^{2}   \\
&\text{s.t.}\quad \mathbf{L} = \sum_{k \in [r]} \sigma_k \mathbf{u}_k \mathbf{v}_k^\top,
\quad \|\mathbf{u}_k\|_\infty \leq \sqrt{\frac{\mu r}{p}}, \|\mathbf{v}_k\|_\infty \leq \sqrt{\frac{\mu r}{q}}
\end{aligned}
\label{eq:tl-step1}
\end{equation}

 
\noindent{\sc Step II.} Use target data to correct mixed estimation. 
\begin{equation}
\begin{aligned}
&\hat{\bD}\in \underset{\bD \in\RR^{p\times q}}{\arg\min}\;  \sum_{i'<i, h\le H}\norm{\phi_{i,h}\psi_{i,h}^\top \bK_{\psi}^{-1} - \phi_{i,h}\phi_{i,h}^\top (\hat\bL + \hat\bS +\bD) }_2^2 \\
&\text{s.t.}\quad \mathbf{L} = \sum_{k \in [r]} \sigma_k \mathbf{u}_k \mathbf{v}_k^\top,
\quad \|\mathbf{u}_k\|_\infty \leq \sqrt{\frac{\mu r}{p}}, \|\mathbf{v}_k\|_\infty \leq \sqrt{\frac{\mu r}{q}}
\end{aligned}
\label{eq:tl-step2}
\end{equation}


\begin{algorithm}
\caption{UCB-TRL(Sparse Matrix Transition Reinforcement Learning)}
\KwIn{Source domain $\mathcal{M}^{(0)}=(\mathcal{S},\mathcal{A},P^{(0)},r,s_0,H)$,\\target domain $\mathcal{M}^{(1)}=(\mathcal{S},\mathcal{A},P^{(1)},r,s_0,H)$,\\
Total number of episode $N_0,N_1$, feature function $\phi\in \mathbb{R}^p, \psi\in \mathbb{R}^q$,\\
Set $L_1,S_1,D_1=\mathbf{0}\in \mathbb{R}^{p\times q}$. 
Empty reply tuple $\mathcal{B}=\emptyset$}
//Estimate the low-rank component\;
\For{episode $i = 1,2,\ldots,N_0$}{    
    Set $Q_{j, h}(s, a)$ in
    (\ref{eq:updateQ}) using $L_j,S_j$  \;
    \For{stage $h = 1,2,\ldots,H$}{
    Take action $a_{i, h}=\arg \max _{a \in \mathcal{A}} Q_{i, h}\left(s_{i, h}, a\right)$\;
    Observe $s_{i, h+1}$ from domain $\mathcal{M}^{(0)}$\;
    %Update dataset $\mathcal{B}=\mathcal{B}\cup \{(s_{i, h}, a_{i, h}, s_{i, h+1})\}$
    }
    Learn transition core $L_i,S_i$ using (\ref{eq:tl-step1}) \\
}
//Use target data to correct mixed estimation\;
\For{episode $j = N_0+1,N_0+2,\ldots,N_0+N_1$}{    
    Set $Q_{j, h}(s, a)$  using $L_j,S_j$  \;
    \For{stage $h = 1,2,\ldots,H$}{
    Take action $a_{j, h}=\arg \max _{a \in \mathcal{A}} Q_{j, h}\left(s_{j, h}, a\right)$\;
    Observe $s_{j, h+1}$ from domain $\mathcal{M}^{(1)}$\;
    Update dataset $\mathcal{B}=\mathcal{B}\cup \{(s_{j, h}, a_{j, h}, s_{j, h+1})\}$
    }
    Learn transition core $L_j,S_j$ using (\ref{eq:tl-step2}) \\
}
\end{algorithm}


Let $N_k$ denote the number of samples in task $k$, $k=0,1$. By Proposition 3 in \citep{basu2019low}, for $N_k$ large enough, \footnote{$N_k \succsim q \paran{\frac{\sup_{\theta \in [-\pi, \pi]}\Lambda_{\max}(f_X(\theta))}{\sup_{\theta \in [-\pi, \pi]}\Lambda_{\min}\paran{f_X(\theta)}}}^2$ where $f_X$ is the spectral density of the VAR model.} there exists a constant $c>0$ such that 
\begin{equation}
\Lambda_{\min}\left(\frac{{\bX^{(k)}}^{\top}\bX^{(k)}}{N_k}\right) \leq c^{(k)},
\label{eq:ass-number}
\end{equation}
    with high probability, \footnote{$1-c_1\exp\paran{-c_2\log p}$ for some constants $c_1, c_2>0$.} Let $\zeta^{(k)}=c^{(k)}$, and then we have the strong convexity condition
    \begin{equation}
    	\frac{1}{2}\norm{\bX^{(k)}\Delta}_F^2 \geq \frac{\zeta^{(k)}}{2}\norm{\bDelta}_F^2, \, \mathrm{for \, all \,} \Delta \in \RR^{p \times q}.
    	\label{eq:StrongConvexity}
    \end{equation}


    The algorithm proceeds in two phases, corresponding to $k \in \{0, 1\}$.
\begin{align*}
Q_{n,h} - \big(r(s_{n,h},a_{n,h}) + [P_h V_{h+1}](s_{n,h},a_{n,h})\big) 
=& \phi_{n, h}^{\top}\left[\left(\widetilde{L}_{n} + \sum_{k=0}^1\widetilde{S}_{n}^{(k)}\right) - M^*\right] \bPsi^{\top} V_{n, h+1} \\
= &\phi_{n, h}^{\top}\left[(\widetilde{L}_{n}-L^*) + \sum_{k=0}^1\left(\widetilde{S}_{n}^{(k)}-S^{*(k)}\right)\right] \bPsi^{\top} V_{n, h+1}.
\end{align*}
The proof is provided in Appendix \ref{A:4}.

In calculating the regret bound, we reformulate the regret formula based on the updates to the Q-values within the algorithm and the confidence bounds of the core matrix. $\mathcal{F}_{n,h}$ is defined as the $\sigma$-field generated by all the random variables up until episode n, step h, essentially fixing the sequence $s_{1,1}, a_{1,1}, s_{1,2}, a_{1,2}, \ldots, s_{n,h}, a_{n,h}$. 
Now, we proceed to prove Theorem \ref{thm:bigtheorem}, letting 
$$\delta_{n,h} := (V_{n,h}-V_{h}^{\pi_{n}})(s_{n,h}), \quad
\gamma_{n,h} := Q_{n,h} - \left(r(s_{n,h},a_{n,h}) + [P_h V_{h+1}](s_{n,h},a_{n,h})\right).$$
\begin{align*}
\text{Regret}(N^{(0)}) &= \mathbb{E}\left(\sum_{n=1}^{N^{(0)}} \left[ V^*(s_0) - V^{\pi_n}(s_0) \right]\right) \\
&\leq \mathbb{E}\left( \sum_{n=1}^{N^{(0)}}(V_{n,1}-V_{1}^{\pi_{n}})(s_0)\right) = \sum_{n=1}^{N^{(0)}}\mathbb{E}(\delta_{n,1}).
\end{align*}
$$\mathbb{E}(\delta_{n,1}) = \mathbb{E}(\delta_{n,1}E_n+(1-E_n)\delta_{n,1}) 
\leq \mathbb{E}(\delta_{n,1}E_n)+Hp[E_n=0].$$
where $p[E_n=0]\leq c_1\exp\paran{-c_2\log p}$, Then we have

\begin{align*}
\mathbb{E}\paran{\delta_{n,1}E_n \mid \mathcal{F}_{n,1}} =& \paran{V_{n,1} - V_{1}^{\pi_{n}}}\paran{s_{n,1}}E_n \\
\leq &Q_{n,1}\paran{s_{n,1},a_{n,1}} - V_{1}^{\pi_{n}}\paran{s_{n,1}} \\
= &\gamma_{n,1} + \paran{r\paran{s_{n,1},a_{n,1}} +[PV_{n,2}]\paran{s_{n,1},a_{n,1}}} -V_{1}^{\pi_{n}}\paran{s_{n,1}} \\
\leq &\gamma_{n,1} + \mathbb{E}\paran{\paran{V_{n,2} - V_{2}^{\pi_{n}}}\paran{s_{n,2}}E_n \mid \mathcal{F}_{n,1}} 
\leq \cdots \leq \sum_{h=1}^{H}\gamma_{n,h}\\
\leq &2C_{\phi}C_{M}C' \sqrt{p}H^2\sqrt{\frac{dr + s\log d}{N_0 + N_1} + \frac{\alpha^2s}{pq}}
\end{align*}



\begin{theorem}
   
$$\norm{\hat\bDelta^L}_F^2+\dfrac{\zeta^{(0)}}{\zeta^{(0)}+ \zeta^{(1)}}\norm{\hat\bDelta^{S, (0)}}_F^2+\dfrac{\zeta^{(1)}}{\zeta^{(0)}+ \zeta^{(1)}}\norm{\hat\bDelta^{S, (1)}}_F^2
    \leq C_2\frac{d+\log d}{N_0+N_1},$$
    with high probability.
    \label{thm:ts-upperbounds2}
   \end{theorem}

   \begin{proof}
   When $K=2$, recall our setting
	$\bY^{(k)} = \bX^{(k)}\paran{\bL+\bS^{*, (k)}} + \bE^{(k)}$, $\bE^{(k)} \overset{\text{i.i.d.}}{\sim} \mathcal{N}\left(0, \Sigma_{\epsilon}\right)$. 
 Analogous to the proof of Theorem\ref{thm:rl-upperbound} for $k \in \braces{0, 1}$, 
           $$\sum_{k=0}^1 \brackets{\frac{1}{2} \norm{\bY^{(k)} - \bX^{(k)} \left( \bL^* + \bS^{*,(k)} + \hat\bDelta^L + \hat\bDelta^{S, (k)} \right)}_F^2} \leq \sum_{k=0}^1 \brackets{\frac{1}{2} \norm{\bY^{(k)} - \bX^{(k)} \left( \bL^* + \bS^{*,(k)} \right)}_F^2}$$
     \begin{equation}		
     \begin{aligned}
     \sum_{k=0}^1 \brackets{\frac{1}{2}\norm{\bX^{(k)}\left(\hat\bDelta^L+\hat\bDelta^{S, (k)}\right)}_F^2}
     & \leq\sum_{k=0}^1 \brackets{\abs{\angles{\paran{\bX^{(k)}}^\top \bE^{(k)},\hat\bDelta^L+\hat\bDelta^{S, (k)}}}}\\
    &\leq \sum_{k=0}^1 \brackets{\norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_2\norm{\hat\bDelta^L}_* + \norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_{\max}\norm{\hat\bDelta^{S, (k)}}_1}
    \end{aligned}
    \label{ineq:difference-Frob2}
    \end{equation}  

    Same to $\hat\bDelta^{S}$, For $k=0,1$, $$\abs{\angles{\hat\bDelta^L,\hat\bDelta^{S, (k)}}}=\abs{\angles{\Pi_J(\hat\bDelta^L),\Pi_J(\hat\bDelta^{S, (k)})}}\leq \norm{\Pi_J(\hat\bDelta^L)}_F^2+\norm{\Pi_J(\hat\bDelta^{S, (k)})}_F^2\leq \frac{1}{4}\paran{\norm{\hat\bDelta^{L}}_F^2+\norm{\hat\bDelta^{S, (k)}}_F^2}$$
     Recalling condition(\ref{ineq:covex-condition}), and inequality(\ref{ineq:lowerbound-Fnorm-XDelta}), we have
     \begin{equation}
     \begin{aligned}
     \sum_{k=0}^1 \brackets{\frac{1}{2}\norm{\bX^{(k)}\left(\hat\bDelta^L+\hat\bDelta^{S, (k)}\right)}_F^2 }&\geq \sum_{k=0}^1 \brackets{\frac{\zeta^{(k)}}{2} \paran{ \norm{\hat\bDelta^L}_F^2 + \norm{\hat\bDelta^{S, (k)}}_F^2 - \abs{\angles{\hat\bDelta^L, \hat\bDelta^{S, (k)}}}}}\\
     &\geq \sum_{k=0}^1 \frac{\zeta^{(k)}}{4} \paran{ \norm{\hat\bDelta^L}_F^2 + \norm{\hat\bDelta^{S, (k)}}_F^2 }
     \end{aligned}
     \end{equation}

     The incoherence property essentially restricts the upper bound of the cross terms in inequality (\ref{ineq:lowerbound-Fnorm-XDelta}). Coupling this with inequality (\ref{ineq:difference-Frob2}), we have,
     \begin{equation}
     \begin{aligned}
      &\sum_{k=0}^1 \frac{\zeta^{(k)}}{4} \paran{ \norm{\hat\bDelta^L}_F^2 + \norm{\hat\bDelta^{S, (k)}}_F^2 }\\
      &\leq \sum_{k=0}^1 \brackets{\norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_2\norm{\hat\bDelta^L}_* + \norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_{\max}\norm{\hat\bDelta^{S, (k)}}_1}\\
      &\leq \sqrt{4\braces{\sum_{k=0}^1\brackets{\frac{\zeta^{(k)}}{4} \paran{\norm{\hat\bDelta^L}_F^2 + \norm{\hat\bDelta^{S, (k)}}_F^2}}}\paran{\norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_2^2+2\norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_{\max}^2}}.
     \end{aligned}
     \end{equation}
     
     By combining lemma \ref{A:3}, which provides upper bounds on 
    $\norm{\bX^{\top}\bE}_2$ and $\norm{\bX^{\top}\bE}_{\max}$, we complete the proof of Theorem \ref{thm:ts-upperbounds2}.

     \begin{equation}
     \begin{aligned}
	 &\quad\norm{\hat\bDelta^L}_F^2+\dfrac{\zeta^{(0)}}{\zeta^{(0)}+ \zeta^{(1)}}\norm{\hat\bDelta^{S, (0)}}_F^2+\dfrac{\zeta^{(1)}}{\zeta^{(0)}+ \zeta^{(1)}}\norm{\hat\bDelta^{S, (1)}}_F^2\\
     &\leq \frac{4}{\zeta^{(0)}+\zeta^{(1)}}\paran{\norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_2^2+2\norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_{\max}^2}
     \leq C_2\frac{d+\log d}{N_0+N_1}.
     \end{aligned}
     \end{equation}

   \end{proof}
   \begin{theorem}
   Given Conditions (\ref{eq:ass-number}) and Conditions in Theorem\ref{thm:ts-upperbounds2}, the cumulative regret of the UCB-TRL algorithm satisfies the following high-probability bound:
    \begin{align*}
    \text{Regret}(N_0)&  \leq 2C_{\phi}C_{M}C_2^{'} \sqrt{pH^3}\sqrt{\frac{N_0^2H}{N_0+N_1}(d+\log d)}\\
    & =\mathcal{O}\paran{C_{\phi}C_{M}C' \sqrt{pH^3}\sqrt{T(d+\log d)}}.
   \end{align*} 
   \end{theorem}




==> macros/algorithm.tex <==


% \usepackage{algorithm,algorithmicx,algpseudocode}
% http://shantoroy.com/latex/how-to-write-algorithm-in-latex/
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}} % require \usepackage{xcolor}
\SetCommentSty{mycommfont}

\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output

==> macros/code.tex <==

%%
%%  code listing macros
%%

%% refs: https://www.overleaf.com/learn/latex/Code_listing

\usepackage{listings}             % Include the listings-package
\lstset{basicstyle=\ttfamily,
	showstringspaces=false,
	commentstyle=\color{red},
	keywordstyle=\color{blue}
}

==> proof.tex <==
\section*{Proof of Theorem \ref{thm:ts-upperbounds}}
	When $K=2$, recall our setting
	$\bY^{(k)} = \bX^{(k)}\bB^{*, (k)} + \bE^{(k)}$, $\bE^{(k)} \overset{\text{i.i.d.}}{\sim} \mathcal{N}\left(0, \Sigma_{\epsilon}\right)$. 
 For $k \in \braces{0, 1}$, where $\bB^{*, (k)} = \bL^* + \bS^{*,(k)}$.
	\begin{gather}
		(\hat\bL, \hat\bS^{(0)}, \hat\bS^{(1)}) 
		= \underset{\bL, \bS, \norm{\bL}_{\max} \leq \frac{\alpha}{p} }{\arg\min}\; \ell\paran{\bL, \bS^{(0)}, \bS^{(1)}}  \nonumber \\
		\ell\paran{\bL, \bS^{(0)}, \bS^{(1)}} 
		\defeq
		\frac{1}{2} \sum_{k=0}^K\norm{\bY^{(k)} - \bX^{(k)}\paran{\bL + \bS^{(k)}}}_F^2
		+ \lam_N \norm{\bL}_* 
		+ \mu^0_{N} \norm{\bS^{(0)}}_1
		+ \mu^1_{N} \norm{\bS^{(1)}}_1. \label{eqn:tl-rank-sparse-K=2}
	\end{gather}
	
	Define $\hat\bDelta^{L}=\hat\bL-\bL^*, \hat\bDelta^{S, (k)}=\hat\bS^{(k)}-\bS^{*, (k)}$. We first show the following lemma, which is adapted from the proof of Lemma 1 in \cite{negahban2012unified}.
	\begin{lemma}
		Suppose $\rank(\bL^*) \leq r$, $\norm{\bS^{*, (k)}}_0 \leq s$ for $k \in \{0, 1\}$, then there exists a decomposition $\hat\bDelta^{L}=\hat\bDelta^{L}_A+ \hat\bDelta^{L}_B$, such that $\rank(\hat\bDelta^{L}_A) \leq 2r$ and
		\begin{equation}
			\norm{\bL^*}_* - \norm{\hat\bL}_* \leq  \norm{\hat\bDelta^{L}_A}_* - \norm{\hat\bDelta^{L}_B}_*.
			\label{ineq:Ldecomp}
		\end{equation}
	   Similarly, there exists a subspace $\calM \subset \RR^{p \times p}$, such that $\norm{\bS^{*, (k)}_{\calM^{\perp}}}_1=0$, and
	    \begin{equation}
	    	\norm{\bS^{*, (k)}}_1 - \norm{\hat\bS^{(k)}}_1 \leq  \norm{\hat\bDelta^{S, (k)}_{\calM}}_1 - \norm{\hat\bDelta^{S, (k)}_{\calM^{\perp}}}_1,
	    	\label{ineq:Sdecomp}
	    \end{equation}
    where $\bA_{\calA}$ stands for the projection of $\bA$ onto subspace $\calA$  and  $\calM^{\perp}$ denotes the orthogonal complement of $\calM$.
	   \label{lem:decomp}
	\end{lemma}
    
    \begin{proof}[Proof of Lemma \ref{lem:decomp}]
    	By in Lemma 3.4 in \cite{recht2010guaranteed}, there exist matrices $\hat\bDelta^{L}_A, \hat\bDelta^{L}_B$ such that
    	$\hat\bDelta^{L}=\hat\bDelta^{L}_A+ \hat\bDelta^{L}_B$, $\rank(\hat\bDelta^{L}_A) \leq 2 \rank(\bL^*) \leq 2r$, and $\paran{\hat\bDelta^{L}_B}^{\top} \bL^* = \bL^* \paran{\hat\bDelta^{L}_B}^{\top} =0$. By Lemma 2.3 in \cite{recht2010guaranteed}, $\norm{\bL^*+\hat\bDelta^{L}_B}_*=\norm{\bL^*}_*+\norm{\hat\bDelta^{L}_B}_*$. Then \eqref{ineq:Ldecomp} holds by
    	$$	\norm{\bL^*}_* - \norm{\hat\bL}_* \leq 	\norm{\bL^*}_* +	\norm{\hat\bDelta^{L}_A}_* -	\norm{\hat\bDelta^{L}_B+\bL^*}_* = \norm{\hat\bDelta^{L}_A}_* - \norm{\hat\bDelta^{L}_B}_*,$$
      where the first inequality comes from triangle inequality. 
      
      For \eqref{ineq:Sdecomp}, take 
      $$\calM = \left\{ (a_{ij}) \in \mathbb{R}^{p \times q} : a_{ij} = 0 \text{ if } \mathbf{S}^{*, (k)}_{ij} = 0 \text{ for both } k = 0 \text{ and } 1 \right\}.$$
     Any matrix in $\calM$ has at most $2s$ nonzero entries, and it's easy to show 
       $$\mathcal{M}^{\perp} = \left\{ (a_{ij}) \in \mathbb{R}^{p \times q} : a_{ij} = 0 \text{ if } \mathbf{S}^{*, (k)}_{ij} \neq 0 \text{ for either } k = 0 \text{ or } 1 \right\}.$$
       
       Therefore,  $\norm{\bS^{*, (k)}_{\calM^{\perp}}}_1=0$, and
       \begin{align*}
       	\norm{\bS^{*, (k)}}_1 - \norm{\hat\bS^{(k)}}_1 &\leq \norm{\bS_\calM^{*, (k)}+\bS_{\calM^\perp}^{*, (k)}}_1 - \norm{\bS^{*, (k)}_\calM + \hat\bDelta^{S,(k)}_{\calM^{\perp}}}_1 + \norm{\hat\bDelta^{S,(k)}_{\calM} + \bS^{*, (k)}_{\calM^{\perp}}}_1\\
       	&\leq \norm{\bS_\calM^{*, (k)}}_1 - \norm{\bS^{*, (k)}_\calM}_1 - \norm{\hat\bDelta^{S,(k)}_{\calM^{\perp}}}_1 + \norm{\hat\bDelta^{S,(k)}_{\calM}}_1 + 2\norm{\bS_{\calM^\perp}^{*, (k)}}_1\\
       	&= \norm{\hat\bDelta^{S,(k)}_{\calM}}_1 - \norm{\hat\bDelta^{S,(k)}_{\calM^{\perp}}}_1.
       \end{align*}
       	\end{proof}
       For $k=0,1$,
       \begin{equation}
       	\begin{aligned}
       		 &\frac{1}{2}\norm{\bY^{(k)}-\bX^{(k)}\left(\bL^*+S^{*,(k)}+\hat\bDelta^L+\hat\bDelta^{S, (k)}\right)}_F^2-      \frac{1}{2}\norm{\bY^{(k)}-\bX^{(k)}\left(\bL^*+S^{*,(k)}\right)}_F^2\\
       		=&\frac{1}{2}\norm{\bX^{(k)}\left(\hat\bDelta^L+\hat\bDelta^{S, (k)}\right)}_F^2-\angles{\bE^{(k)},\bX^{(k)}\left(\hat\bDelta^L+\hat\bDelta^{S, (k)}\right)}\\
       		\geq&\frac{1}{2}\norm{\bX^{(k)}\paran{\hat\bDelta^L+\hat\bDelta^{S, (k)}}}_F^2-\abs{\angles{\paran{\bX^{(k)}}^\top \bE^{(k)},\hat\bDelta^L+\hat\bDelta^{S, (k)}}}\\
       		\geq & \frac{1}{2}\norm{\bX^{(k)}\paran{\hat\bDelta^L+\hat\bDelta^{S, (k)}}}_F^2 - \norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_2\norm{\hat\bDelta^L}_* - \norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_{\max}\norm{\hat\bDelta^{S, (k)}}_1\\
       		\geq &\frac{1}{2}\norm{\bX^{(k)}\paran{\hat\bDelta^L+\hat\bDelta^{S, (k)}}}_F^2 - \frac{\lambda_N}{4}\norm{\hat\bDelta^L}_* - \frac{\mu^k_N}{2}\norm{\hat\bDelta^{S, (k)}}_1.
       	\end{aligned}
       \label{ineq:difference-Frob}
       \end{equation}
       The second last inequality holds because $\|\cdot\|_{2}$ and $\|\cdot\|_{*}$ are dual norms, so do $\|\cdot\|_{\max}$ and $\|\cdot\|_{1}$. The last inequality comes from our assumptions about $\lambda_N$ and $\mu^k_N$. By inequality \eqref{ineq:difference-Frob} and Lemma \ref{lem:decomp}, 
        \begin{equation}
       	\begin{aligned}
       		 &\ell(\hat\bL, \hat\bS^{(0)}, \hat\bS^{(1)}) - \ell(\bL^*, \bS^{*,(0)}, \bS^{*,(1)})\\
       		=&\sum_{k=0}^1\brackets{\frac{1}{2} \norm{\bY^{(k)}-\bX^{(k)}\left(\bL^*+\bS^{*,(k)}+\hat\bDelta^L+\hat\bDelta^{S, (k)}\right)}_F^2-      \frac{1}{2}\norm{\bY^{(k)}-\bX^{(k)}\left(\bL^*+\bS^{*,(k)}\right)}_F^2}\\
       		+&\lambda_N\paran{\norm{\hat\bL}_*-\norm{\bL^*}_*} + \sum_{k=0}^1 \mu^k_{N}\brackets{\norm{\hat\bS^{(k)}}_1-\norm{\bS^{*, (k)}}_1}\\
       		\geq&\sum_{k=0}^1\brackets{\frac{1}{2}\norm{\bX^{(k)}\left(\hat\bDelta^L+\hat\bDelta^{S, (k)}\right)}_F^2-\frac{\lambda_N}{4}\norm{\hat\bDelta^L}_* - \frac{\mu^k_N}{2}\norm{\hat\bDelta^{S, (k)}}_1} - \lambda_N\paran{\norm{\hat\bDelta^{L}_A}_* - \norm{\hat\bDelta^{L}_B}_*} \\
       		- & \sum_{k=0}^1 \mu^k_{N}\brackets{\norm{\hat\bDelta^{S, (k)}_{\calM}}_1 - \norm{\hat\bDelta^{S, (k)}_{\calM^{\perp}}}_1}.
       	\end{aligned}
        \label{ineq:difference-l}
       \end{equation}
       	Since $\ell(\hat\bL, \hat\bS^{(0)}, \hat\bS^{(1)}) - \ell(\bL^*, \bS^{(0), *}, \bS^{(1), *})\leq 0$, we obtain 
       	$$-\lambda_N\paran{\norm{\hat\bDelta^{L}_A}_* - \norm{\hat\bDelta^{L}_B}_*} - \sum_{k=0}^1 \mu^k_{N}\brackets{\norm{\hat\bDelta^{S, (k)}_{\calM}}_1 - \norm{\hat\bDelta^{S, (k)}_{\calM^{\perp}}}_1} \leq \frac{\lambda_N}{2}\norm{\hat\bDelta^L}_* + \sum_{k=0}^1 \frac{\mu^k_N}{2}\norm{\hat\bDelta^{S, (k)}}_1,$$
       	which implies that
       	\begin{equation}
       		\lambda_N\norm{\hat\bDelta^{L}_B}_* + \sum_{k=0}^1\mu^k_N\norm{\hat\bDelta^{S, (k)}_{\calM^{\perp}}}_1 \leq 3\paran{\lambda_N\norm{\hat\bDelta^{L}_A}_* + \sum_{k=0}^1\mu^k_N\norm{\hat\bDelta^{S, (k)}_{\calM}}_1},
       		\label{ineq:BMcleq3AM}
       	\end{equation}
       and hence
      \begin{equation}
       	 \sum_{k=0}^1\mu^k_N\norm{\hat\bDelta^{S, (k)}}_1 \leq 3\lambda_N\norm{\hat\bDelta^{L}_A}_* + 4 \sum_{k=0}^1\mu^k_N\norm{\hat\bDelta^{S, (k)}_{\calM}}_1.
       	\label{ineq:DeltaSleq3A+4M}
       \end{equation}
       Also by \eqref{ineq:difference-l}, 
       \begin{equation}
       	\sum_{k=0}^1\brackets{\frac{1}{2}\norm{\bX^{(k)}\left(\hat\bDelta^L+\hat\bDelta^{S, (k)}\right)}_F^2} \leq \frac{3}{2}\paran{\lambda_N\norm{\hat\bDelta^{L}_A}_* + \sum_{k=0}^1\mu^k_N\norm{\hat\bDelta^{S, (k)}_{\calM}}_1}.
       	\label{ineq:upperbound-Fnorm-XDelta}
       \end{equation}
	  Since with high probability,
	   $$\Lambda_{\min}\paran{\paran{\bX^{(k)}}^{\top}\bX^{(k)}} < \zeta^{(k)},$$
	   $\Lambda_{\min}$ represents the minimum eigenvalue of a matrix. we have
       \begin{equation}
	   \frac{1}{2}\norm{\bX^{(k)}\left(\hat\bDelta^L+\hat\bDelta^{S, (k)}\right)}_F^2 \geq \frac{\zeta^{(k)}}{2} \norm{\hat\bDelta^L+\hat\bDelta^{S, (k)}}^2_F,
       \label{ineq:covex-condition}
       \end{equation}
	    with high probability. Note that 
	    \begin{equation}
	    	    \begin{aligned}
	    		\norm{\hat\bDelta^L+\hat\bDelta^{S, (k)}}^2_F&\geq \norm{\hat\bDelta^L}_F^2 + \norm{\hat\bDelta^{S, (k)}}_F^2 - \abs{\angles{\hat\bDelta^L, \hat\bDelta^{S, (k)}}}\\
	    		&\geq \norm{\hat\bDelta^L}_F^2 + \norm{\hat\bDelta^{S, (k)}}_F^2  
	    		-\norm{\hat\bDelta^L}_{\max} \norm{\hat\bDelta^{S, (k)}}_1\\
	    		&\geq \norm{\hat\bDelta^L}_F^2 + \norm{\hat\bDelta^{S, (k)}}_F^2-\frac{2\alpha}{p}\norm{\hat\bDelta^{S, (k)}}_1\\
	    		&\geq \norm{\hat\bDelta^L}_F^2 + \norm{\hat\bDelta^{S, (k)}}_F^2-\frac{\mu_N^k}{\zeta^{(k)}}\norm{\hat\bDelta^{S, (k)}}_1,
	    	\end{aligned}
    	\label{ineq:lowerbound-Fnorm-XDelta}
	    \end{equation}
	   where the second-to-last inequality holds because both $\norm{\bL^*}_{\max} \leq \frac{\alpha}{p}$ and $\norm{\hat \bL}_{\max} \leq \frac{\alpha}{p}$, and the last inequality comes from our choice of $\mu_N^k$. Combining \eqref{ineq:lowerbound-Fnorm-XDelta}, \eqref{ineq:upperbound-Fnorm-XDelta} and \eqref{ineq:DeltaSleq3A+4M} yields that
	   \begin{equation}
	   	\begin{aligned}
	   			   	&\quad\sum_{k=0}^1\brackets{\frac{\zeta^{(k)}}{2} \paran{\norm{\hat\bDelta^L}_F^2 + \norm{\hat\bDelta^{S, (k)}}_F^2}}\\ & \leq \sum_{k=0}^1 \frac{\mu_N^k}{2}\norm{\hat\bDelta^{S, (k)}}_1 + \frac{3}{2}\paran{\lambda_N\norm{\hat\bDelta^{L}_A}_* + \sum_{k=0}^1\mu^k_N\norm{\hat\bDelta^{S, (k)}_{\calM}}}_1\\
	   			   	&\leq 3\lambda_N\norm{\hat\bDelta^{L}_A}_* + \frac{7}{2} \sum_{k=0}^1\mu^k_N\norm{\hat\bDelta^{S, (k)}_{\calM}}_1\\
	   			   	&\leq 3\lambda_N\sqrt{2r}\norm{\hat\bDelta^{L}}_F+ \frac{7}{2}\sqrt{2s} \sum_{k=0}^1\mu^k_N\norm{\hat\bDelta^{S, (k)}}_F\\
	   			   	&\leq \sqrt{\braces{\sum_{k=0}^1\brackets{\frac{\zeta^{(k)}}{2} \paran{\norm{\hat\bDelta^L}_F^2 + \norm{\hat\bDelta^{S, (k)}}_F^2}}}\paran{\frac{36\lambda_N^2 r}{\zeta^{(0)}+\zeta^{(1)}}+\frac{49(\mu^0_N)^2 s}{\zeta^{(0)}}+\frac{49(\mu^1_N)^2 s}{\zeta^{(1)}}}}.
	   	\end{aligned}
	   \end{equation}
	   Therefore,
	  \begin{equation}
	   	\begin{aligned}
	   		&\quad\norm{\hat\bDelta^L}_F^2+\dfrac{\zeta^{(0)}}{\zeta^{(0)}+ \zeta^{(1)}}\norm{\hat\bDelta^{S, (0)}}_F^2+\dfrac{\zeta^{(1)}}{\zeta^{(0)}+ \zeta^{(1)}}\norm{\hat\bDelta^{S, (1)}}_F^2\\
	   		&\leq \frac{2}{\zeta^{(0)}+\zeta^{(1)}}\paran{\frac{36\lambda_N^2 r}{\zeta^{(0)}+\zeta^{(1)}}+\frac{49(\mu^0_N)^2 s}{\zeta^{(0)}}+\frac{49(\mu^1_N)^2 s}{\zeta^{(1)}}}.
	   	\end{aligned}
	   \end{equation}

\section*{Proof of Theorem \ref{thm:ts-upperbounds2}}      
     $$\sum_{k=0}^1 \brackets{\frac{1}{2} \norm{\bY^{(k)} - \bX^{(k)} \left( \bL^* + \bS^{*,(k)} + \hat\bDelta^L + \hat\bDelta^{S, (k)} \right)}_F^2} \leq \sum_{k=0}^1 \brackets{\frac{1}{2} \norm{\bY^{(k)} - \bX^{(k)} \left( \bL^* + \bS^{*,(k)} \right)}_F^2}$$
     \begin{equation}		
     \begin{aligned}
     \sum_{k=0}^1 \brackets{\frac{1}{2}\norm{\bX^{(k)}\left(\hat\bDelta^L+\hat\bDelta^{S, (k)}\right)}_F^2}
     & \leq\sum_{k=0}^1 \brackets{\abs{\angles{\paran{\bX^{(k)}}^\top \bE^{(k)},\hat\bDelta^L+\hat\bDelta^{S, (k)}}}}\\
    &\leq \sum_{k=0}^1 \brackets{\norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_2\norm{\hat\bDelta^L}_* + \norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_{\max}\norm{\hat\bDelta^{S, (k)}}_1}
    \end{aligned}
    \label{ineq:difference-Frob2}
    \end{equation}  
    
    By the separation lemma presented in \cite{chai2024structured}, this lemma demonstrates that two matrices can be well-separated to a certain extent under the incoherence assumption. Given two $\mu'$-incoherent matrices $G_1,G_2\in \RR^{p \times q}$, with $\mu'$ having an upper bound $\mu$, and $\rank(G_1),\rank(G_2)\leq r$. Let $\bDelta^G=G_1-G_2$, we have $\frac{\norm{\bDelta^G}^2_{max}}{\norm{\bDelta^G}_F^2}\leq \frac{c\mu r^4}{\max\{p,q\}}$, 
    
    Define the support sets of matrices $\hat\bDelta^{L}$ and $\hat\bDelta^{S, (k)}$ as $ \text{supp}(\hat\bDelta^{L})=\{(i,j)\mid \hat\bDelta^{L}_{i,j}\neq 0\}$ and $\text{supp}(\hat\bDelta^{S, (k)})\{(i,j)\mid \hat\bDelta^{S, (k)}_{i,j}\neq 0\}$, respectively, and let $J = \text{supp}(\hat\bDelta^{L}) \cap \text{supp}(\hat\bDelta^{S, (k)})$. The projection operator $\Pi_J$ zeros out elements not in $J$. Hence,$$\frac{\norm{\Pi_J(\hat\bDelta^{L})}_F^2}{\norm{\hat\bDelta^{L}}_F^2}\leq |J|\frac{\norm{\hat\bDelta^{L}}_{max}^2}{\norm{\hat\bDelta^{L}}_F^2}\leq 2s\frac{c\mu r^4}{\max\{p,q\}}\leq \frac{\max\{p,q\}}{8c\mu r^4}\frac{c\mu r^4}{\max\{p,q\}}=\frac{1}{4}$$
    Same to $\hat\bDelta^{S, (k)}$, For $k=0,1$, $$\abs{\angles{\hat\bDelta^L,\hat\bDelta^{S, (k)}}}=\abs{\angles{\Pi_J(\hat\bDelta^L),\Pi_J(\hat\bDelta^{S, (k)})}}\leq \norm{\Pi_J(\hat\bDelta^L)}_F^2+\norm{\Pi_J(\hat\bDelta^{S, (k)})}_F^2\leq \frac{1}{4}\paran{\norm{\hat\bDelta^{L}}_F^2+\norm{\hat\bDelta^{S, (k)}}_F^2}$$
     Recalling condition(\ref{ineq:covex-condition}), and inequality(\ref{ineq:lowerbound-Fnorm-XDelta}), we have
     \begin{equation}
     \begin{aligned}
     \sum_{k=0}^1 \brackets{\frac{1}{2}\norm{\bX^{(k)}\left(\hat\bDelta^L+\hat\bDelta^{S, (k)}\right)}_F^2 }&\geq \sum_{k=0}^1 \brackets{\frac{\zeta^{(k)}}{2} \paran{ \norm{\hat\bDelta^L}_F^2 + \norm{\hat\bDelta^{S, (k)}}_F^2 - \abs{\angles{\hat\bDelta^L, \hat\bDelta^{S, (k)}}}}}\\
     &\geq \sum_{k=0}^1 \frac{\zeta^{(k)}}{4} \paran{ \norm{\hat\bDelta^L}_F^2 + \norm{\hat\bDelta^{S, (k)}}_F^2 }
     \end{aligned}
     \end{equation}

     The incoherence property essentially restricts the upper bound of the cross terms in inequality (\ref{ineq:lowerbound-Fnorm-XDelta}). Coupling this with inequality (\ref{ineq:difference-Frob2}), we have,
     \begin{equation}
     \begin{aligned}
      &\sum_{k=0}^1 \frac{\zeta^{(k)}}{4} \paran{ \norm{\hat\bDelta^L}_F^2 + \norm{\hat\bDelta^{S, (k)}}_F^2 }\\
      &\leq \sum_{k=0}^1 \brackets{\norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_2\norm{\hat\bDelta^L}_* + \norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_{\max}\norm{\hat\bDelta^{S, (k)}}_1}\\
      &\leq \sqrt{4\braces{\sum_{k=0}^1\brackets{\frac{\zeta^{(k)}}{4} \paran{\norm{\hat\bDelta^L}_F^2 + \norm{\hat\bDelta^{S, (k)}}_F^2}}}\paran{\norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_2^2+2\norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_{\max}^2}}.
     \end{aligned}
     \end{equation}
     
     By combining lemma \ref{A:3}, which provides upper bounds on 
    $\norm{\bX^{\top}\bE}_2$ and $\norm{\bX^{\top}\bE}_{\max}$, we complete the proof of Theorem \ref{thm:ts-upperbounds2}.

     \begin{equation}
     \begin{aligned}
	 &\quad\norm{\hat\bDelta^L}_F^2+\dfrac{\zeta^{(0)}}{\zeta^{(0)}+ \zeta^{(1)}}\norm{\hat\bDelta^{S, (0)}}_F^2+\dfrac{\zeta^{(1)}}{\zeta^{(0)}+ \zeta^{(1)}}\norm{\hat\bDelta^{S, (1)}}_F^2\\
     &\leq \frac{4}{\zeta^{(0)}+\zeta^{(1)}}\paran{\norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_2^2+2\norm{\paran{\bX^{(k)}}^\top \bE^{(k)}}_{\max}^2}
     \leq C_2\frac{d+\log d}{N_0+N_1}.
     \end{aligned}
     \end{equation}

 \section*{Proof of Lemma \ref{lem:xe-bound}}
 \label{A:3}
Building upon the research presented in \cite{basu2015regularized} and \cite{basu2019low}, deviation bounds for $\norm{\bX^{\top}E}_2$ and $\norm{\bX^{\top}E}_{\max}$have been established for the regularized estimation of low-dimensional structures. The transition core matrix is not necessarily square, we extend of Proposition 3 from \cite{basu2019low},  derive the following results:
\begin{lemma}
Let $X \in \mathbb{R}^{p \times p}$ and $E \in \mathbb{R}^{p \times q}$, denote $d = \max\{p,q\}$, satisfying the settings in (1). There exist positive constants $c_1$ and $c_2$ such that,\\
for $N \gtrsim d$, 
 $$\mathbb{P}\left( \left\| \frac{X^\top E}{N} \right\|_2 > c_0 \varphi(B, \Sigma_{\epsilon})\sqrt{\frac{d}{N}} \right) \leq c_1 \exp \left[-c_2 \log p\right],$$
and for any  $N \gtrsim \log d$, 
$$\mathbb{P}\left( \left\| \frac{X^\top E}{N} \right\|_{\max} > c_0 \varphi(B, \Sigma_{\epsilon})\sqrt{\frac{\log d}{N}} \right) \leq c_1 \exp \left[-c_2 \log p\right]$$
\label{lem:xe-bound}
\end{lemma}

\begin{proof}
 Without loss of generality, assume that $p > q$. We augment the matrix $E \in \mathbb{R}^{p \times q}$ to a $p \times p$ matrix form $E' = [E, \mathbf{0}_{p,p-q}]$. $\norm{X^{\top}E'}_2\leq \norm{X^{\top}E}_2,\norm{X^{\top}E}_{\max}\leq \norm{X^{\top}E'}_{\max}$. We can now directly apply Proposition 3 in \cite{basu2019low} to the pair $(X, E')$.
\   
\end{proof}
 
\section*{Proof of Lemma \ref{lem:boundQ} } 
\label{A:4}
\begin{proof}
        Applying Hölder's inequality, the triangle inequality, and Cauchy-Schwarz inequality, we deduce the following results:
     \begin{equation}
     \begin{aligned}
     &Q_{n,h} - \left(r + [P_h V_{h+1}]\right) \\
     &\leq \norm{\phi_{n, h}^{\top}(\widetilde{\bL}_{n} - \bL^{*})}_*\norm{\bPsi^{\top} V_{n, h+1}}_{op}+\sum_{k=0}^1\norm{\phi_{n, h}^{\top}\paran{\widetilde{\bS}_{n} - \bS^{(1)}}}_1\norm{\bPsi^{\top} V_{n, h+1}}_{\infty} \\
     & \leq \paran{C_{\psi,1}\norm{\phi_{n, h}^{\top}(\widetilde{\bL}_{n} - \bL^*)}_*+C_{\psi,2}\sum_{k=0}^1\norm{\phi_{n, h}^{\top}\paran{\widetilde{\bS}_{n}^{(k)} - \bS^{*(k)}}}_1}H \\
     & \leq \paran{C_{\psi,1}\sqrt{2r}\norm{\phi_{n, h}^{\top}}_*\norm{\widetilde{\bL}_{n} - \bL^{*}}_F + C_{\psi,2}\sqrt{s}\sum_{k=0}^1\norm{\phi_{n, h}^{\top}}_1\norm{\widetilde{\bS}_{n}^{(k)} - \bS^{*(k)}}_F}H \\
     & \leq C_{\phi}\sqrt{p}H\paran{C_{\psi,1}\sqrt{2r}\norm{\widetilde{\bL}_{n} - \bL^*}_F + C_{\psi,2}\sqrt{s}\sum_{k=0}^1
     \norm{\widetilde{\bS}_{n}^{(k)} - \bS^{*(k)}}_F} \\
     & \leq C_{\phi}\sqrt{p}H \sqrt{2rC_{\psi,1}^2 \|\widetilde{\bL}_{n} - \bL^*\|_F^2 + sC_{\psi,2}^2 \sum_{k=0}^1 \|\widetilde{\bS}_{n}^{(k)} - \bS^{*(k)}\|_F^2}\\
     & \overset{(1)}{\leq}C_{\phi}C_{M}\sqrt{p}H
     \sqrt{
     \norm{\widetilde{\bL}_n -\hat\bL_n}^2_F + 
     \norm{\hat\bL_n -\bL^*}^2_F+\sum_{k=0}^1\paran{\norm{\widetilde{\bS}_{n}^{(k)} - \hat\bS_n^{(k)}}^2_F+\norm{\hat\bS_n^{(k)} - S^{*(k)}}^2_F}} \\
     & \leq 2C_{\phi}C_{M}C^{'} \sqrt{p}H\sqrt{\frac{dr+s\log d}{N_0+N_1}+\frac{\alpha^2s}{pq}}
     \end{aligned}
    \end{equation}
\end{proof}

Inequality $(1)$ holds because $\|\widetilde{\bL}_{n} - \bL^*\|_F^2 + \sum_{k=0}^1 \|\widetilde{\bS}_{n}^{(k)} - \bS^{*(k)}\|_F^2 \leq C$, Constants $2rC_{\psi,1}^2$ and $sC_{\psi,2}^2$ are subsumed under the maximum operation to form the consolidated constant term $C_M$ for brevity.
 
    
   

==> self-defined.tex <==
% Copy right @ 2019
% All right reserved by Elynn Y. Chen.
% This file defines short-hands for math formulas.
% It started with  Prof. Jianqing Fan's macro definition.
% Later it incorporated some of my own macro definition.
%
%
% Other references:
% -- math guide: http://mirrors.rit.edu/CTAN/info/short-math-guide/short-math-guide.pdf
% -- bold math symbol: https://tex.stackexchange.com/questions/595/how-can-i-get-bold-math-symbols
%
%

\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}
\renewcommand{\bar}{\overline}

%--------------------------------
%
%  Boldfaces in Letters
%
% \newcommand{\bfm}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\bfm}[1]{\ensuremath{\boldsymbol{#1}}} % bm

\def\bzero{\bfm 0}
\def\bone{\bfm 1}
\def\bbone{\mathbbm{1}} % package bm

\def\ba{\bfm a}   \def\bA{\bfm A}  \def\AA{\mathbb{A}}
\def\bb{\bfm b}   \def\bB{\bfm B}  \def\BB{\mathbb{B}}
\def\bc{\bfm c}   \def\bC{\bfm C}  \def\CC{\mathbb{C}}
\def\bd{\bfm d}   \def\bD{\bfm D}  \def\DD{\mathbb{D}}
\def\be{\bfm e}   \def\bE{\bfm E}  \def\EE{\mathbb{E}}
\def\bff{\bfm f}  \def\bF{\bfm F}  \def\FF{\mathbb{F}}
\def\bg{\bfm g}   \def\bG{\bfm G}  \def\GG{\mathbb{G}}
\def\bh{\bfm h}   \def\bH{\bfm H}  \def\HH{\mathbb{H}}
\def\bi{\bfm i}   \def\bI{\bfm I}  \def\II{\mathbb{I}}
\def\bj{\bfm j}   \def\bJ{\bfm J}  \def\JJ{\mathbb{J}}
\def\bk{\bfm k}   \def\bK{\bfm K}  \def\KK{\mathbb{K}}
\def\bl{\bfm l}   \def\bL{\bfm L}  \def\LL{\mathbb{L}}
\def\bm{\bfm m}   \def\bM{\bfm M}  \def\MM{\mathbb{M}}
\def\bn{\bfm n}   \def\bN{\bfm N}  \def\NN{\mathbb{N}}
\def\bo{\bfm o}   \def\bO{\bfm O}  \def\OO{\mathbb{O}}
\def\bp{\bfm p}   \def\bP{\bfm P}  \def\PP{\mathbb{P}}
\def\bq{\bfm q}   \def\bQ{\bfm Q}  \def\QQ{\mathbb{Q}}
\def\br{\bfm r}   \def\bR{\bfm R}  \def\RR{\mathbb{R}}
\def\bs{\bfm s}   \def\bS{\bfm S}  \def\SS{\mathbb{S}}
\def\bt{\bfm t}   \def\bT{\bfm T}  \def\TT{\mathbb{T}}
\def\bu{\bfm u}   \def\bU{\bfm U}  \def\UU{\mathbb{U}}
\def\bv{\bfm v}   \def\bV{\bfm V}  \def\VV{\mathbb{V}}
\def\bw{\bfm w}   \def\bW{\bfm W}  \def\WW{\mathbb{W}}
\def\bx{\bfm x}   \def\bX{\bfm X}  \def\XX{\mathbb{X}}
\def\by{\bfm y}   \def\bY{\bfm Y}  \def\YY{\mathbb{Y}}
\def\bz{\bfm z}   \def\bZ{\bfm Z}  \def\ZZ{\mathbb{Z}}

\def\calA{{\cal  A}} \def\cA{{\cal  A}}
\def\calB{{\cal  B}} \def\cB{{\cal  B}}
\def\calC{{\cal  C}} \def\cC{{\cal  C}}
\def\calD{{\cal  D}} \def\cD{{\cal  D}}
\def\calE{{\cal  E}} \def\cE{{\cal  E}}
\def\calF{{\cal  F}} \def\cF{{\cal  F}}
\def\calG{{\cal  G}} \def\cG{{\cal  G}}
\def\calH{{\cal  H}} \def\cH{{\cal  H}}
\def\calI{{\cal  I}} \def\cI{{\cal  I}}
\def\calJ{{\cal  J}} \def\cJ{{\cal  J}}
\def\calK{{\cal  K}} \def\cK{{\cal  K}}
\def\calL{{\cal  L}} \def\cL{{\cal  L}}
\def\calM{{\cal  M}} \def\cM{{\cal  M}}
\def\calN{{\cal  N}} \def\cN{{\cal  N}}
\def\calO{{\cal  O}} \def\cO{{\cal  O}}
\def\calP{{\cal  P}} \def\cP{{\cal  P}}
\def\calQ{{\cal  Q}} \def\cQ{{\cal  Q}}
\def\calR{{\cal  R}} \def\cR{{\cal  R}}
\def\calS{{\cal  S}} \def\cS{{\cal  S}}
\def\calT{{\cal  T}} \def\cT{{\cal  T}}
\def\calU{{\cal  U}} \def\cU{{\cal  U}}
\def\calV{{\cal  V}} \def\cV{{\cal  V}}
\def\calW{{\cal  W}} \def\cW{{\cal  W}}
\def\calX{{\cal  X}} \def\cX{{\cal  X}}
\def\calY{{\cal  Y}} \def\cY{{\cal  Y}}
\def\calZ{{\cal  Z}} \def\cZ{{\cal  Z}}

\def\calh{{\cal h}}

%--------------------------------
%
%  Boldfaces in Greek
%
\newcommand{\bfsym}[1]{\ensuremath{\boldsymbol{#1}}}

 \def\balpha{\bfsym \alpha}
 \def\bbeta{\bfsym \beta}
 \def\bgamma{\bfsym \gamma}             \def\bGamma{\bfsym \Gamma}
 \def\bdelta{\bfsym {\delta}}           \def\bDelta {\bfsym {\Delta}}
 \def\bfeta{\bfsym {\eta}}              \def\bfEta {\bfsym {\Eta}}
 \def\bmu{\bfsym {\mu}}                 \def\bMu {\bfsym {\Mu}}
 \def\bnu{\bfsym {\nu}}
 \def\btheta{\bfsym {\theta}}           \def\bTheta {\bfsym {\Theta}}
 \def\beps{\bfsym \varepsilon}          \def\bEps{\bfsym{\mathcal E}}
 \def\bepsilon{\bfsym \varepsilon}
 \def\bsigma{\bfsym \sigma}             \def\bSigma{\bfsym \Sigma}
  \def\bsig{\bfsym \sigma}             \def\bSig{\bfsym \Sigma}
 \def\blambda {\bfsym {\lambda}}        \def\bLambda {\bfsym {\Lambda}}
 \def\bomega {\bfsym {\omega}}          \def\bOmega {\bfsym {\Omega}}
 \def\brho   {\bfsym {\rho}}
 \def\btau{\bfsym {\tau}}
 \def\bxi{\bfsym {\xi}}          \def\bXi{\bfsym {\Xi}}
 \def\bzeta{\bfsym {\zeta}}
 \def\bpi{\bfsym {\pi}}          \def\bPi{\bfsym {\Pi}}
\def\bphi{\bfsym {\phi}}          \def\bPhi{\bfsym {\Phi}}
\def\bpsi{\bfsym {\psi}}          \def\bPsi{\bfsym {\Psi}}
\def\bchi{\bfsym {\chi}}          \def\bChi{\bfsym {\Chi}}
\def\bupsi{\bfsym {\upsilon}}          \def\bUpsi{\bfsym {\Upsilon}}

 %--------------------------------
 %
 %  Hat (boldface) in Greek
 %
  \def\halpha{\hat{\alpha}}              \def\hbalpha{\hat{\bfsym \alpha}}
  \def\hbeta{\hat{\beta}}                \def\hbbeta{\hat{\bfsym \beta}}
  \def\hgamma{\hat{\gamma}}              \def\hgamma{\hat{\bfsym \gamma}}
  \def\hGamma{\hat{ \Gamma}}             \def\hbGamma{\hat{\bfsym \Gamma}}
  \def\hdelta{\hat{\delta}}              \def\hbdelta{\hat{\bfsym {\delta}}}
  \def\hDelta {\hat{\Delta}}             \def\hbDelta{\hat{\bfsym {\Delta}}}
  \def\heta{\hat {\eta}}                 \def\hbfeta {\hat{\bfsym {\eta}}}
  \def\hmu{\hat{\mu}}                    \def\hbmu {\hat{\bfsym {\mu}}}
  \def\hnu{\hat{\nu}}                    \def\hbnu {\hat{\bfsym {\nu}}}
  \def\htheta{\hat {\theta}}             \def\hbtheta {\hat{\bfsym {\theta}}}
  \def\hTheta{\hat {\Theta}}             \def\hbTheta {\hat{\bfsym {\Theta}}}
  \def\hbeps{\hat{\bfsym \varepsilon}}   \def\hbepsilon{\hat{\bfsym \varepsilon}}
  \def\hsigma{\hat{\sigma}}              \def\hbsigma{\hat{\bfsym \sigma}}
  \def\hSigma{\hat{\Sigma}}              \def\hbSigma{\hat{\bfsym \Sigma}}
  \def\hlambda{\hat{\lambda}}            \def\hblambda{\hat{\bfsym \lambda}}
  \def\hLambda{\hat{\Lambda}}            \def\hbLambda{\hat{\bfsym \Lambda}}
  \def\homega {\hat {\omega}}            \def\hbomega {\hat{\bfsym {\omega}}}
  \def\hOmega {\hat {\omega}}            \def\hbOmega {\hat{\bfsym {\Omega}}}
  \def\hrho   {\hat {\rho}}              \def\hbrho {\hat{\bfsym {\rho}}}
  \def\htau   {\hat {\tau}}              \def\hbtau {\hat{\bfsym {\tau}}}
  \def\hxi{\hat{\xi}}                    \def\hbxi{\hat{\bfsym {\xi}}}
  \def\hzeta{\hat{\zeta}}                \def\hbzeta{\hat{\bfsym {\bzeta}}}


 %--------------------------------
 %
 %  Operator
 %
\providecommand{\abs}[1]{\left\lvert#1\right\rvert}
\providecommand{\norm}[1]{\left\lVert#1\right\rVert}

\providecommand{\angles}[1]{\left\langle #1 \right\rangle}
\providecommand{\paran}[1]{\left( #1 \right)}
\providecommand{\brackets}[1]{\left[ #1 \right]}
\providecommand{\braces}[1]{\left\{ #1 \right\}}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\providecommand{\convprob}{\stackrel{\calP}{\longrightarrow}}
\providecommand{\convdist}{\stackrel{\calD}{\longrightarrow}}
\providecommand{\defeq}{\triangleq}
% \providecommand{\defeq}{\dot{=}}

\usepackage{mathtools}
% K-L divergence
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1 \; \delimsize\| \; #2%
}
\newcommand{\infdiv}{\calD \infdivx}
\newcommand{\kldiv}{\calD_{KL} \infdivx}

%--------------------------------
%
% Regular font in math equation
%

\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\corr}{corr}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Dev}{Dev}
\DeclareMathOperator{\diag}{diag}
%\DeclareMathOperator{\E}{E}
\newcommand{\E}[1]{{\mathbb{E}} \left[ #1 \right]}
\DeclareMathOperator{\logit}{logit}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\RSS}{RSS}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\SE}{SE}
\DeclareMathOperator{\Prob}{Pr}
%\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
%\DeclareMathOperator{\vect}{vec}
\newcommand{\vect}[1]{{\textsc{vec}} \left( #1 \right)}
\newcommand{\mat}[1]{{\textsc{mat}} \left( #1 \right)}


%--------------------------------
%
%  Thms, Props, Assumps, Remarks, et al
%

%\newtheorem{definition}{Definition}[section]
%\newtheorem{assumption}[definition]{Assumption}
%\newtheorem{lemma}[definition]{Lemma}
%\newtheorem{proposition}[definition]{Proposition}
%\newtheorem{theorem}[definition]{Theorem}
%\newtheorem{corollary}[definition]{Corollary}
%\newtheorem{exercise}[definition]{Exercise}
%\newtheorem{example}[definition]{Example}
%
%\newenvironment{solution}{\paragraph{Solution:}}{\hfill$\square$}
%
%\renewcommand*{\theassumption}{\Alph{assumption}}

% \newtheorem{definition}{Definition}
% \newtheorem{assumption}{Assumption}
% \newtheorem{lemma}{Lemma}
% \newtheorem{proposition}{Proposition}
% \newtheorem{theorem}{Theorem}
% \newtheorem{corollary}{Corollary}

%\def\remark{{\noindent\underbar{\bf Remark}\quad}}
%\newtheorem{remark}{Remark}

%--------------------------------
%
%  Bachmann-Landau or asymptotic notations
%
% determiniastic convergence
\newcommand{\bigO}[1]{ \mathcal{O} \left( #1 \right) }
\newcommand{\bigOmega}[1]{ \Omega \left( #1 \right) }
\newcommand{\bigTheta}[1]{ \Theta \left( #1 \right) }
\newcommand{\smlo}[1]{{\rm o} \left( #1 \right) }
\newcommand{\smlomega}[1]{{\omega} \left( #1 \right) }

% converge in probability
\newcommand{\Op}[1]{{\mathcal{O}_p} \left( #1 \right) }
\newcommand{\op}[1]{{\rm o_p} \left( #1 \right) }

%--------------------------------
%
%  Markers
%
% need \usepackage[table,xcdraw,dvipsnames]{xcolor}   % for \textcolor

% colorful text emphasizer
\providecommand{\textem}[1]{\textit{\textcolor{Cerulean}{#1}}}

% comments
\definecolor{royalpurple}{rgb}{0.47, 0.32, 0.66}
\providecommand{\elynn}[1]{\textcolor{RubineRed}{\bf [Elynn: #1]}}
\providecommand{\attn}[1]{\textcolor{red}{\bf (#1)}}
\providecommand{\xuening}[1]{\textcolor{blue}{\bf [Xuening: #1]}}

 %--------------------------------
%
%  Semi-parametric specials
%

\newcommand{\jbracket}[1]{ J_{[]}\braces{#1} }
\newcommand{\nbracket}[1]{ N_{[]}\braces{#1} }

 %--------------------------------
 %
 %  Shorthands
 %

\def\eps{\varepsilon}
\def\lam {\lambda}
\def\blam {\blambda}
\def\bLam {\bLambda}
\def\bdiag{{\rm bdiag}}

\def\vec{\mbox{vec}}
\def\wh{\widehat}
\def\blue{\color{blue}}
\def\red{\color{red}}

% May add more in future.

\newenvironment{question}{ \color{teal} \textbf{To settle:}  }{\hfill$\clubsuit$}

